Parallel Dynamic Maximal Matching

We present the first (randomized) parallel dynamic algorithm for maximal matching, which can process an arbitrary number of updates simultaneously. Given a batch of edge deletion or insertion updates to the graph, our parallel algorithm adjusts the maximal matching to these updates in $poly(\log n)$ depth and using $poly(\log n)$ amortized work per update. That is, the amortized work for processing a batch of $k$ updates is $kpoly(\log n)$, while all this work is done in $poly(\log n)$ depth, with high probability. This can be seen as a parallel counterpart of the sequential dynamic algorithms for constant-approximate and maximal matching [Onak and Rubinfeld STOC'10; Baswana, Gupta, and Sen FOCS'11; and Solomon FOCS'16]. Our algorithm readily generalizes to maximal matching in hypergraphs of rank $r$ -- where each hyperedge has at most $r$ endpoints -- with a $poly(r)$ increase in work, while retaining the $poly(\log n)$ depth.

==> Reviewer_Comments.tex <==
Reviewer A:

p.3: at this point in the paper, it is unclear what the second property means. 

> Done

p.4: S_\ell -> S?

> Done

p.4: the intuition behind temporarily deleted edges was hard to understand.

> Added a little more? But it's hard to see what exactly is unclear

p.5: it might be better to use different notation than O(v) and O(e), to avoid confusion with big oh notation.

> No, because it's notation from all previous paper, and it would be even more confusing

p.6: how does B differ from S_\ell?

> Done

p.7: The "a"s in the proof of Theorem 4.4 should be "alpha"s.

> Done

Reviewer D: 

You are missing big-O notation in a number of places when talking about runtimes (e.g., when talking about the Brent's scheduling principle).

> Everything seems fine to me in that paragraph

Prior to Theorem 2.2 M was defined as the size of the batch (in Theorem 1.1). You might want to be consistent with your variable names to avoid confusing the reader.

> In 1.1:  $M$ denotes the total number of hyperedges inserted or deleted (starting from an empty graph).

In 2.2:  Here, $M$ denotes the total number of hyperedges.

I think it's reasonable to denote total numbers of edges in graphs as $M$ in both cases (even though in the first case it's more like number of operations)
